Boosting Inference Efficiency: Unleashing the Power of Parameter-Shared Pre-trained Language Models

Parameter-shared pre-trained language models (PLMs) have emerged as a successful approach in resource-constrained environments, enabling substantial reductions in model storage and memory costs without significant performance compromise. However, it is important to note that parameter sharing does not alleviate computational burdens associated with inference, thus impeding its practicality in situations characterized by limited stringent latency requirements or computational resources. Building upon neural ordinary differential equations (ODEs), we introduce a straightforward technique to enhance the inference efficiency of parameter-shared PLMs. Additionally, we propose a simple pre-training technique that leads to fully or partially shared models capable of achieving even greater inference acceleration. The experimental results demonstrate the effectiveness of our methods on both autoregressive and autoencoding PLMs, providing novel insights into more efficient utilization of parameter-shared models in resource-constrained settings.

==> figs_code/bert-other.tex <==
\begin{figure*}[ht!]
    \centering
    \subfloat[MNLI]{\includegraphics[width=0.33\textwidth]{figs/bert-search-mnli.pdf}}
\hfill
    \subfloat[SST-2]{\includegraphics[width=0.33\textwidth]{figs/bert-search-sst2.pdf}}
\hfill
    \subfloat[SQuAD]{\includegraphics[width=0.33\textwidth]{figs/bert-search-squad.pdf}}
    \caption{The inference performance of parameter-shared BERT models with reduced number of layers and scaled-up step size on MNLI, SST-2 and SQuAD.}
    \label{fig:gamma1-performance-add}
\end{figure*}

==> figs_code/gamma1-performance-other.tex <==
\begin{figure*}[ht!]
    \centering
% \hfill
    % \subfloat[MNLI]{\includegraphics[width=0.245\textwidth]{figs/bert-search-mnli.pdf}}
% \hfill
    \subfloat[SST-2]{\includegraphics[width=0.245\textwidth]{figs/bert-search-sst2.pdf}}
% \hfill
%     \subfloat[RACE]{\includegraphics[width=0.245\textwidth]{figs/bert-search-race.pdf}}
% \hfill
    \subfloat[SQuAD]{\includegraphics[width=0.245\textwidth]{figs/bert-search-squad.pdf}}
% \hfill
    \subfloat[SQuAD2.0]{\includegraphics[width=0.245\textwidth]{figs/bert-search-squad2.pdf}}
% \hfill
%     \subfloat[LAMBADA]{\includegraphics[width=0.245\textwidth]{figs/gpt-search-lambada.pdf}}
% \hfill
%     \subfloat[Wikitext-103]{\includegraphics[width=0.245\textwidth]{figs/gpt-search-wiki.pdf}}
% \hfill
    % \caption{The inference performance of parameter-shared models pre-trained with different step size. (a-e) The accuracy of BERT on MNLI, SST-2, RACE and the F1 score on SQuAD and SQuAD2.0. (f-g) The zero-shot accuracy of GPT-2 on LAMBADA, and the zero-shot perplexity of GPT-2 on Wikitext-103.}
    \caption{The inference performance of parameter-shared BERT pre-trained with different step size. We report the accuracy for SST-2, and F1 score for SQuAD and SQuAD2.0.}
    \label{fig:gamma1-performance-other}
\end{figure*}

==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

==> tables_code/bert-search.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l r r r r r}
\toprule
Model & MNLI & SST-2 & RACE & SQuAD & SQuAD 2.0\\
\midrule
\multicolumn{2}{l}{\textit{24 Layers}}\\
BERT$_\text{large}$-1 & 83.6 & 90.6 & 63.9 & 90.1 & 81.2\\
BERT$_\text{large}$-0.1 & 83.2 & 91.4 & 67.5 & 90.1 & 81.4\\
BERT$_\text{large}$-0.01 & 81.7 & 90.1 & 64.4 & 89.3 & 79.5\\
Hyper BERT$_\text{large}$-0.1 & 85.7 & 93.1 & 71.7 & 91.2 & 82.0\\
\midrule
\multicolumn{2}{l}{\textit{12 Layers}}\\
BERT$_\text{base}$ (no sharing) & 84.4 & 92.7 & 67.2 & 90.4 & 80.2\\
BERT$_\text{large}$-1 & 81.1 & 90.4 & 59.4 & 83.0 & 65.0\\
BERT$_\text{large}$-0.1 & 81.2 & 89.8 & 60.7 & 83.4 & 70.0\\
BERT$_\text{large}$-0.01 & 82.3 & 91.1 & 62.9 & 87.4 & 75.7\\
Hyper BERT$_\text{large}$-0.1 & 83.8 & 92.5 & 65.0 & 89.2 & 78.0\\
\bottomrule
\end{tabular}
\caption{}
\end{table*}

==> tables_code/bert.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l r r r r r}
\toprule
Model & MNLI & SST-2 & RACE & SQuAD & SQuAD 2.0\\
\midrule
\multicolumn{2}{l}{\textit{24 Layers}}\\
BERT$_\text{large}$-1 & 83.6 & 90.6 & 64.3 & 90.1 & 81.4\\
BERT$_\text{large}$-0.1 & 83.2 & 91.4 & 67.5 & 90.1 & 81.4\\
BERT$_\text{large}$-0.01 & 81.7 & 90.5 & 64.4 & 89.3 & 79.5\\
Hyper BERT$_\text{large}$-0.1 & 85.7 & 93.1 & 71.7 & 91.2 & 82.0\\
\midrule
\multicolumn{2}{l}{\textit{12 Layers}}\\
BERT$_\text{base}$ (no sharing) & 84.4 & 92.7 & 67.2 & 90.4 & 80.2\\
BERT$_\text{large}$-1 & 72.0 & 86.6 & 52.3 & 62.3 & 33.8\\
BERT$_\text{large}$-0.1 & 57.4 & 85.3 & 49.8 & 61.0 & 46.5\\
BERT$_\text{large}$-0.01 & 82.0 & 90.6 & 62.7 & 86.2 & 73.2\\
Hyper BERT$_\text{large}$-0.1 & 83.5 & 90.6 & 62.8 & 87.9 & 74.7\\
\bottomrule
\end{tabular}
\caption{}
\end{table*}

==> tables_code/downstream-config-0.01.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l r r r r r}
    \toprule
    \textbf{Hyper-Parameter} & \textbf{MNLI} & \textbf{SST-2} &\textbf{RACE} & \textbf{SQuAD} & \textbf{SQuAD2} \\
    \midrule
	lr & 4e-05 & 2e-05 & 3e-05 & 2e-05 & 3e-05 \\ 
	iterations & 12270 & 12627 & 21964 & 16452 & 8160 \\ 
	batch size & 64 & 16 & 16 & 16 & 32 \\ 
	warmup ratio & 0.05 & 0.01 & 0.01 & 0.05 & 0.01 \\ 
    \bottomrule
    \end{tabular}
    \caption{Hyper-parameters for downstream tasks with step size = 0.01.}
    \label{tab:hyperparameter-step-0.01}
\end{table*}

==> tables_code/downstream-config-0.05.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l r r r r r}
    \toprule
    \textbf{Hyper-Parameter} & \textbf{MNLI} & \textbf{SST-2} &\textbf{RACE} & \textbf{SQuAD} & \textbf{SQuAD2} \\
    \midrule
	lr & 1e-05 & 3e-05 & 2e-05 & 3e-05 & 2e-05 \\ 
	iterations & 98172 & 10520 & 13725 & 8226 & 32640 \\ 
	batch size & 16 & 32 & 32 & 32 & 16 \\ 
	warmup ratio & 0.1 & 0.05 & 0.1 & 0.01 & 0.01 \\ 
    \bottomrule
    \end{tabular}
    
    \caption{Hyper-parameters for downstream tasks with step size = 0.05.}
    \label{tab:hyperparameter-step-0.05}
\end{table*}

==> tables_code/downstream-config-0.1.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l r r r r r}
    \toprule
    \textbf{Hyper-Parameter} & \textbf{MNLI} & \textbf{SST-2} &\textbf{RACE} & \textbf{SQuAD} & \textbf{SQuAD2} \\
    \midrule
	lr & 1e-05 & 1e-05 & 2e-05 & 3e-05 & 2e-05 \\ 
	iterations & 98172 & 6312 & 27455 & 8226 & 20400 \\ 
	batch size & 16 & 32 & 16 & 32 & 32 \\ 
	warmup ratio & 0.1 & 0.1 & 0.05 & 0.1 & 0.1 \\ 
    \bottomrule
    \end{tabular}
    
    \caption{Hyper-parameters for downstream tasks with step size = 0.1.}
    \label{tab:hyperparameter-step-0.1}
\end{table*}

==> tables_code/downstream-config-1.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l r r r r r}
    \toprule
    \textbf{Hyper-Parameter} & \textbf{MNLI} & \textbf{SST-2} &\textbf{RACE} & \textbf{SQuAD} & \textbf{SQuAD2} \\
    \midrule
    lr & 2e-05 & 1e-05 & 1e-05 & 3e-05 & 2e-05 \\ 
	iterations & 30675 & 10520 & 27455 & 8226 & 20400 \\ 
	batch size & 64 & 32 & 16 & 32 & 32 \\ 
	warmup ratio & 0.05 & 0.01 & 0.1 & 0.01 & 0.01 \\ 
    \bottomrule
    \end{tabular}
    
    \caption{Hyper-parameters for downstream tasks with step size = 1.}
    \label{tab:hyperparameter-step-1}
\end{table*}


==> tables_code/downstream-config-mnli.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l l l l l}
    \toprule
    \textbf{Step Size} & \textbf{1} & \textbf{0.1} & \textbf{0.05} & \textbf{0.01}\\
    \midrule
    lr & 2e-5 & 1e-5 & 1e-5 & 4e-5\\
    lr decay style & linear & linear & linear & linear\\
    min lr & 0.0 & 0.0 & 0.0 & 0.0 \\
    iterations & 30,675 & 98,172 & 98,172 & 12,270\\
    batch size & 64 & 16 & 16 & 64 \\
    weight decay & 0.01 & 0.01 & 0.01 & 0.01 \\
    warmup ratio & 0.05 & 0.1 & 0.1 & 0.05 \\
    gradient norm & 1.0 & 1.0 & 1.0 & 1.0\\
    dropout & 0.1 & 0.1 & 0.1 & 0.1 \\
    \bottomrule
    \end{tabular}
    \caption{Hyper-parameters for the MNLI downstream task in this work.}
    \label{tab:bert-config}
\end{table}



==> tables_code/optimal-step-scales.tex <==
\begin{table*}[ht!]
\centering
\resizebox{\textwidth}{!}{
% \scriptsize
\tiny
\setlength{\defaultaddspace}{1pt} 
\setlength{\cmidrulewidth}{0.01em} 
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.8} % Default value: 1
\begin{tabular}{c c l}
\toprule
\textbf{Step Size} & \textbf{Iterate Time} & \multicolumn{1}{c}{\textbf{Optimal Step Sizes}} \\
\midrule
\multicolumn{3}{c}{MNLI} \\
\cmidrule(lr{7pt}){1-3}
1 & 12 & 1.0,1.2,1.7,2.3,1.5,1.2,1.6,2.1,1.6,2.7,2.0,2.8\\ 
  & 16 & 1.4,1.1,1.5,1.9,2.7,2.1,1.1,2.3,1.2,2.4,3.0,2.9,1.6,2.5,1.5,2.7\\ 
  & 20 & 1.3,1.0,1.7,1.5,2.0,2.3,1.4,1.8,1.4,1.6,1.4,1.4,1.2,1.2,2.2,1.3,1.9,2.3,1.4,1.1\\ 
0.1 & 12 & 1.0,1.1,1.2,2.9,1.2,1.6,1.9,1.3,2.4,2.4,2.6,1.8\\ 
  & 16 & 1.0,1.1,1.3,1.2,1.4,1.1,2.4,1.5,2.6,1.9,2.6,1.8,1.1,2.5,1.8,3.0\\ 
  & 20 & 1.0,1.1,1.8,1.1,1.4,1.9,2.9,1.1,1.7,1.2,1.0,1.2,1.0,1.3,1.4,1.6,1.3,1.1,1.4,1.0\\ 
0.05 & 12 & 1.7,1.4,1.5,2.8,1.3,1.3,2.8,1.9,2.2,1.3,2.9,2.7\\ 
  & 16 & 1.0,1.7,1.1,2.8,1.4,1.8,2.0,3.0,1.4,1.8,2.0,2.5,1.4,1.7,1.4,2.7\\ 
  & 20 & 1.1,2.3,1.7,2.4,2.0,2.3,1.8,1.1,2.2,2.0,2.1,1.2,2.3,2.0,1.7,1.9,1.8,1.0,1.5,1.0\\ 
0.01 & 12 & 2.1,1.3,2.5,1.2,1.9,1.9,1.5,2.6,1.5,1.3,2.1,2.7\\ 
  & 16 & 1.0,2.8,1.3,1.2,3.0,1.2,1.4,1.7,3.0,1.1,1.5,2.2,1.5,1.4,2.1,1.3\\ 
  & 20 & 1.0,2.2,1.4,2.3,2.4,1.5,1.0,2.3,3.0,2.7,1.9,2.2,1.8,1.0,1.1,1.5,1.5,1.5,1.2,1.2\\ 
\cmidrule(lr{7pt}){1-3}
\multicolumn{3}{c}{SST-2} \\
\cmidrule(lr{7pt}){1-3}
1 & 12 & 1.1,1.3,2.0,1.7,1.3,1.7,1.5,1.7,1.1,1.3,2.5,2.9\\ 
  & 16 & 1.3,1.2,2.7,2.1,1.1,1.2,2.7,1.9,1.6,1.1,1.7,1.1,2.3,1.2,2.7,1.5\\ 
  & 20 & 1.1,1.0,1.0,1.3,1.0,1.0,1.6,1.1,1.0,1.4,1.0,1.1,1.1,1.3,1.0,1.0,1.0,1.5,1.0,1.0\\ 
0.1 & 12 & 1.2,1.4,2.0,1.0,2.1,1.1,1.3,2.0,1.0,3.0,2.9,2.5\\ 
  & 16 & 1.2,1.0,1.1,1.0,1.4,2.4,1.0,1.5,1.1,1.8,1.8,2.2,2.6,2.6,2.7,2.0\\ 
  & 20 & 1.2,1.0,1.1,1.0,2.7,1.1,1.1,1.4,2.2,1.2,1.0,1.6,2.6,1.3,1.0,2.0,1.5,1.2,2.5,2.8\\ 
0.05 & 12 & 1.2,1.3,1.4,1.0,1.3,1.1,2.9,1.0,1.6,2.5,3.0,2.4\\ 
  & 16 & 1.1,1.3,1.1,1.9,1.1,1.1,2.0,1.3,1.7,1.5,1.0,2.6,1.9,2.9,1.1,2.6\\ 
  & 20 & 1.3,1.2,1.0,1.2,1.2,1.2,1.0,1.5,1.4,1.5,1.9,1.1,1.4,2.9,2.8,2.2,1.2,1.9,1.5,2.1\\ 
0.01 & 12 & 1.0,1.0,1.3,2.3,2.2,1.0,2.8,1.3,1.9,1.3,1.7,1.8\\ 
  & 16 & 2.3,1.0,1.1,2.3,2.1,1.8,2.0,2.0,1.6,1.8,3.0,1.0,2.7,1.8,1.4,1.2\\ 
  & 20 & 1.2,1.3,1.4,1.0,1.7,1.4,2.9,2.7,2.7,1.1,1.2,2.7,2.7,1.3,2.6,2.2,2.1,1.3,2.8,2.0\\ 
\cmidrule(lr{7pt}){1-3}
\multicolumn{3}{c}{RACE} \\
\cmidrule(lr{7pt}){1-3}
1 & 12 & 1.0,1.0,1.1,1.1,1.1,1.0,1.3,1.6,2.1,2.0,2.8,2.9\\ 
  & 16 & 1.1,1.1,1.9,1.4,1.7,1.1,1.6,1.5,1.0,1.3,2.0,1.1,3.0,1.6,1.4,2.2\\ 
  & 20 & 1.1,2.1,1.0,1.5,1.1,2.3,1.2,1.0,1.1,1.0,1.3,1.2,1.8,1.3,1.6,1.3,1.7,1.1,2.2,1.4\\ 
0.1 & 12 & 1.1,1.0,1.2,2.1,1.3,1.6,2.1,1.3,2.8,1.5,3.0,2.7\\ 
  & 16 & 1.0,1.1,1.3,2.4,1.5,1.0,1.3,3.0,1.0,1.7,1.5,1.1,1.7,2.8,3.0,1.4\\ 
  & 20 & 1.0,1.2,1.0,1.4,1.0,1.0,1.0,2.0,1.2,1.3,1.5,1.1,2.2,1.5,1.1,1.2,1.0,1.3,1.2,1.5\\ 
0.05 & 12 & 1.4,1.3,1.1,2.1,1.0,1.4,1.2,2.9,1.4,2.9,2.4,2.5\\ 
  & 16 & 1.2,1.4,1.0,1.6,1.7,1.0,3.0,1.4,1.6,2.1,2.3,1.7,1.9,1.6,1.3,1.1\\ 
  & 20 & 1.2,1.2,1.7,1.0,2.9,1.0,1.6,1.3,1.8,1.1,2.2,1.9,1.0,2.9,2.1,1.1,1.0,1.1,1.5,2.3\\ 
0.01 & 12 & 1.2,1.5,1.1,2.6,1.1,1.5,1.5,2.9,1.9,1.3,2.8,3.0\\ 
  & 16 & 1.0,2.1,1.1,1.7,1.3,2.1,1.5,2.1,2.1,1.4,2.9,1.1,1.0,1.0,2.0,2.8\\ 
  & 20 & 1.2,1.1,1.1,1.0,2.1,1.5,2.0,1.9,1.2,1.8,2.3,1.5,2.2,1.4,3.0,1.2,1.0,1.0,1.5,1.5\\
\cmidrule(lr{7pt}){1-3}
\multicolumn{3}{c}{SQuAD} \\
\cmidrule(lr{7pt}){1-3}
1 & 12 & 1.0,1.1,1.4,1.6,1.4,1.6,1.6,1.8,1.4,2.9,3.0,2.7\\ 
  & 16 & 1.1,1.3,1.7,1.5,1.3,1.7,1.6,1.9,1.4,1.8,2.5,1.7,2.5,2.3,2.7,2.7\\ 
  & 20 & 1.1,1.7,1.3,1.3,1.4,1.0,1.6,1.4,1.8,1.2,1.0,1.7,1.3,1.6,1.3,1.8,1.8,1.5,2.4,1.1\\ 
0.1 & 12 & 1.1,1.0,1.4,1.9,1.4,1.2,1.2,1.9,2.3,2.4,2.0,3.0\\ 
  & 16 & 1.0,1.1,1.6,1.1,1.3,1.8,1.2,1.2,2.7,1.4,1.8,2.5,1.3,1.6,2.5,2.1\\ 
  & 20 & 1.1,1.0,1.2,1.4,1.0,1.4,2.3,1.2,1.8,2.2,2.0,1.3,1.1,1.6,1.3,1.1,1.4,1.5,1.1,1.1\\ 
0.05 & 12 & 1.3,1.7,1.4,1.6,1.1,2.7,1.1,2.1,1.3,2.8,2.6,3.0\\ 
  & 16 & 1.2,1.1,1.8,1.3,1.6,2.1,1.3,2.3,1.9,1.5,1.0,1.5,1.8,1.6,1.5,2.4\\ 
  & 20 & 1.3,1.1,1.7,1.0,1.3,1.6,1.0,1.1,1.3,1.3,1.1,2.2,1.4,1.1,1.2,1.3,1.1,1.0,2.6,1.0\\ 
0.01 & 12 & 1.4,1.7,1.9,1.2,2.0,1.5,1.4,1.5,2.6,1.8,2.7,3.0\\ 
  & 16 & 1.7,1.1,1.6,1.4,2.2,1.2,2.3,1.0,1.2,1.7,1.4,1.2,1.7,1.5,1.7,1.7\\ 
  & 20 & 1.3,1.6,1.1,1.9,1.1,1.3,1.7,1.1,1.3,1.1,1.0,1.0,1.1,1.0,1.3,1.2,1.3,1.2,1.2,1.2\\ 
\cmidrule(lr{7pt}){1-3}
\multicolumn{3}{c}{SQuAD2} \\
\cmidrule(lr{7pt}){1-3}
1 & 12 & 1.0,1.5,1.5,1.3,1.5,2.6,2.1,1.7,2.8,2.5,1.8,2.9\\ 
  & 16 & 1.0,1.9,1.4,1.7,1.3,1.3,1.7,1.7,1.5,2.1,1.9,1.6,2.2,2.8,3.0,2.6\\ 
  & 20 & 1.0,1.6,1.2,1.1,1.1,1.0,1.3,1.1,1.7,1.0,2.6,1.2,1.6,1.0,1.5,1.1,1.2,1.8,1.8,1.6\\ 
0.1 & 12 & 1.0,1.2,1.4,1.8,2.4,1.4,1.2,1.9,2.4,2.8,3.0,2.8\\ 
  & 16 & 1.0,1.1,1.4,1.5,1.4,1.7,2.5,1.6,2.4,1.1,2.0,1.2,2.5,1.1,1.9,2.7\\ 
  & 20 & 1.0,1.0,1.2,1.0,1.0,1.3,2.4,2.0,1.3,1.2,1.6,1.0,1.3,1.1,1.3,1.2,2.5,2.4,1.2,1.2\\ 
0.05 & 12 & 1.2,1.2,2.9,1.1,2.2,1.4,1.4,1.6,2.9,2.4,2.8,2.9\\ 
  & 16 & 1.4,1.2,1.7,1.5,1.3,2.0,1.0,2.0,1.8,1.5,1.0,1.6,2.2,1.0,3.0,2.9\\ 
  & 20 & 1.0,2.1,1.0,1.9,1.0,1.0,1.0,1.3,1.1,1.0,1.3,1.0,1.0,1.4,1.6,1.2,1.1,1.1,1.2,1.1\\ 
0.01 & 12 & 1.7,1.1,2.6,1.2,2.1,1.5,1.1,3.0,1.3,2.4,3.0,2.6\\ 
  & 16 & 1.8,1.0,1.1,2.0,1.1,2.4,1.6,2.1,1.1,1.0,1.7,1.1,2.2,1.1,1.3,1.3\\ 
  & 20 & 1.5,1.0,1.1,2.0,1.4,2.2,1.7,1.9,1.4,1.1,1.0,1.3,1.2,1.3,1.2,1.0,1.6,1.1,1.7,1.4\\
\bottomrule
\end{tabular}
}
\caption{Hyper-parameters for downstream tasks with step size = 0.01.}
\label{tab:bert-config}
\end{table*}

==> tables_code/step-size-1-search.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l *{7}{r@{}l}}
\toprule
 & \multicolumn{10}{c}{\textbf{BERT}} & \multicolumn{4}{c}{\textbf{GPT-2}}\\
\cmidrule(lr){2-11} \cmidrule(lr){12-15}
\textbf{\#Iters} & \multicolumn{2}{c}{\textbf{MNLI$\uparrow$}} & \multicolumn{2}{c}{\textbf{SST-2$\uparrow$}} & \multicolumn{2}{c}{\textbf{RACE$\uparrow$}} & \multicolumn{2}{c}{\textbf{SQuAD$\uparrow$}} & \multicolumn{2}{c}{\textbf{SQuAD2$\uparrow$}} & \multicolumn{2}{c}{\textbf{Wiki-103$\downarrow$}} & \multicolumn{2}{c}{\textbf{LAMBADA$\uparrow$}}\\
\midrule

\bottomrule
\end{tabular}
\caption{}
\label{}
\end{table*}
